Ab-initio Contrast Estimation and Denoising of Cryo-EM Images

Background and Objective: The contrast of cryo-EM images varies from one to another, primarily due to the uneven thickness of the ice layer. This contrast variation can affect the quality of 2-D class averaging, 3-D ab-initio modeling, and 3-D heterogeneity analysis. Contrast estimation is currently performed during 3-D iterative refinement. As a result, the estimates are not available at the earlier computational stages of class averaging and ab-initio modeling. This paper aims to solve the contrast estimation problem directly from the picked particle images in the ab-initio stage, without estimating the 3-D volume, image rotations, or class averages. Methods: The key observation underlying our analysis is that the 2-D covariance matrix of the raw images is related to the covariance of the underlying clean images, the noise variance, and the contrast variability between images. We show that the contrast variability can be derived from the 2-D covariance matrix and we apply the existing Covariance Wiener Filtering (CWF) framework to estimate it. We also demonstrate a modification of CWF to estimate the contrast of individual images. Results: Our method improves the contrast estimation by a large margin, compared to the previous CWF method. Its estimation accuracy is often comparable to that of an oracle that knows the ground truth covariance of the clean images. The more accurate contrast estimation also improves the quality of image restoration as demonstrated in both synthetic and experimental datasets. Conclusions: This paper proposes an effective method for contrast estimation directly from noisy images without using any 3-D volume information. It enables contrast correction in the earlier stage of single particle analysis, and may improve the accuracy of downstream processing.

==> Contrast Estimation 3DEM_arXiv/macro_file.tex <==
%&LaTeX

%%% This document contains macros that will be used throughout
%%% It is very neatly organized.


%%%%% Packages

%\usepackage[notcite]{showkeys}

\usepackage{amsthm}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{bm}
\usepackage{mathrsfs}

\usepackage{algorithm}
\usepackage{algorithmic}

\usepackage{color}
\usepackage[dvipsnames]{xcolor}

\usepackage{url}
%\usepackage{citesort}

\usepackage{supertabular}

%\usepackage{enumitem}

\newcommand{\tm}[1]{{\leavevmode\color{RawSienna}{[TM] #1}}}


%%% Theorem setup

%\theoremstyle{plain}

\newtheoremstyle{mystyle}%                % Name
  {}%                                     % Space above
  {}%                                     % Space below
  {\itshape}%                                     % Body font
  {}%                                     % Indent amount
  {\bfseries}%                            % Theorem head font
  {.}%                                    % Punctuation after theorem head
  { }%                                    % Space after theorem head, ' ', or \newline
  {}%                                     % Theorem head spec (can be left empty, meaning `normal')

\theoremstyle{mystyle}
\newtheorem{lemma}{Lemma}
\newtheorem{example}{Example}
\newtheorem{proposition}{Proposition}

\newtheorem{bigthm}{Theorem}
\renewcommand{\thebigthm}{\Alph{bigthm}}	% Number with A, B, C, etc.

\newtheorem{thm}{Theorem}
\newtheorem{cor}[thm]{Corollary}
%\newtheorem{lemma}[thm]{Lemma}
\newtheorem{prop}[thm]{Proposition}

\theoremstyle{definition}
\newtheorem{defn}[thm]{Definition}

%\newtheorem{algorithm}[thm]{Algorithm}

\theoremstyle{remark}

\newtheorem{fact}[thm]{Fact}
\newtheorem{claim}[thm]{Claim}

\newtheorem{rem}[thm]{Remark}



%\newtheorem{example}[thm]{Example}


%\newtheorem*{notation}{Notation}

%\numberwithin{equation}%{section}

\numberwithin{thm}{section}

%\numberwithin{figure}{chapter}
%\numberwithin{table}{chapter}


%%% Typesetting

\DeclareMathAlphabet{\mathsfsl}{OT1}{cmss}{m}{sl}


%%% Other font changes

\newcommand{\lang}{\textit}
\newcommand{\titl}{\textsl}
\newcommand{\term}{\emph}

%\newcommand{\algname}{\textsc}

\newcommand{\notate}[1]{\textcolor{red}{\textbf{[#1]}}}
\newcommand{\marginnote}[1]{\marginpar{\tiny{\notate{#1}}}}
\newcommand{\cnst}[1]{\mathrm{#1}}


%%% Old symbols with new names

\newcommand{\oldphi}{\phi}
\renewcommand{\phi}{\varphi}

\newcommand{\eps}{\varepsilon}


%%% New symbols

\newcommand{\defby}{\overset{\mathrm{\scriptscriptstyle{def}}}{=}}
\newcommand{\half}{\tfrac{1}{2}}
\newcommand{\third}{\tfrac{1}{3}}

\newcommand{\sumnl}{\sum\nolimits}
\newcommand{\defeq}{\mathrel{\mathop{:}}=}
\newcommand{\latop}[2]{\genfrac{}{}{0pt}{}{#1}{#2}}


%%% Constants

\newcommand{\econst}{\mathrm{e}}
\newcommand{\iunit}{\mathrm{i}}

\newcommand{\onevct}{\mathbf{e}}
\newcommand{\zerovct}{\vct{0}}

%\newcommand{\Id}{\mathsf{I}}
%\newcommand{\onemtx}{\mathsf{1}}
%\newcommand{\zeromtx}{\mathsf{0}}

\newcommand{\Id}{\mathbf{I}}
\newcommand{\onemtx}{\bm{1}}
\newcommand{\zeromtx}{\bm{0}}


%%% Sets

\newcommand{\coll}[1]{\mathscr{#1}}

\newcommand{\Sspace}[1]{\mathbb{S}^{#1}}

\newcommand{\Rplus}{\mathbb{R}_{+}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\C}{\mathbb{C}}

\newcommand{\M}{\mathbb{M}}


%%% Real and complex analysis

\newcommand{\abs}[1]{\left\vert {#1} \right\vert}
\newcommand{\abssq}[1]{{\abs{#1}}^2}

\newcommand{\sgn}[1]{\operatorname{sgn}{#1}}
\newcommand{\real}{\operatorname{Re}}
\newcommand{\imag}{\operatorname{Im}}

\newcommand{\diff}[1]{\mathrm{d}{#1}}
\newcommand{\idiff}[1]{\, \diff{#1}}

\newcommand{\grad}{\nabla}
\newcommand{\subdiff}{\partial}

\newcommand{\argmin}{\operatorname*{arg\,min}}
\newcommand{\argmax}{\operatorname*{arg\,max}}


%%% Probability

\newcommand{\Probe}[1]{\mathbb{P}\left({#1}\right)}
\newcommand{\Prob}[1]{\mathbb{P}\left\{ {#1} \right\}}
\newcommand{\Expect}{\operatorname{\mathbb{E}}}

\newcommand{\normal}{\textsc{normal}}
\newcommand{\erf}{\operatorname{erf}}



%%% Vector and matrix operators

\newcommand{\vct}[1]{\bm{#1}}
\newcommand{\mtx}[1]{\bm{#1}}
\newcommand{\tvct}[1]{\tilde{\vct{#1}}} % Add tilde to vector
%\newcommand{\mtx}[1]{\mathsfsl{#1}}

%\newcommand{\transp}{\mathrm{T}}
\newcommand{\transp}{*}
\newcommand{\adj}{*}
\newcommand{\psinv}{\dagger}

\newcommand{\lspan}[1]{\operatorname{span}{#1}}

\newcommand{\range}{\operatorname{range}}
\newcommand{\colspan}{\operatorname{colspan}}

\newcommand{\rank}{\operatorname{rank}}

\newcommand{\diag}{\operatorname{diag}}
\newcommand{\trace}{\operatorname{tr}}

\newcommand{\supp}[1]{\operatorname{supp}(#1)}

\newcommand{\smax}{\sigma_{\max}}
\newcommand{\smin}{\sigma_{\min}}

% Projection operator
\newcommand{\Proj}{\ensuremath{\mtx{\Pi}}}

%%% Semidefinite orders

\newcommand{\psdle}{\preccurlyeq}
\newcommand{\psdge}{\succcurlyeq}

\newcommand{\psdlt}{\prec}
\newcommand{\psdgt}{\succ}

%%% Mensuration: inner products and norms

\newcommand{\ip}[2]{\left\langle {#1},\ {#2} \right\rangle}
\newcommand{\absip}[2]{\abs{\ip{#1}{#2}}}
\newcommand{\abssqip}[2]{\abssq{\ip{#1}{#2}}}
\newcommand{\tworealip}[2]{2 \, \real{\ip{#1}{#2}}}

\newcommand{\norm}[1]{\left\Vert {#1} \right\Vert}
\newcommand{\normsq}[1]{\norm{#1}^2}

% Fixed-size inner products and norms are useful sometimes

\newcommand{\smip}[2]{\bigl\langle {#1}, \ {#2} \bigr\rangle}
\newcommand{\smabsip}[2]{\bigl\vert \smip{#1}{#2} \bigr\vert}
\newcommand{\smnorm}[2]{{\bigl\Vert {#2} \bigr\Vert}_{#1}}

% Specific norms that are used frequently

\newcommand{\enorm}[1]{\norm{#1}}
\newcommand{\enormsq}[1]{\enorm{#1}^2}

\newcommand{\fnorm}[1]{\norm{#1}_{\mathrm{F}}}
\newcommand{\fnormsq}[1]{\fnorm{#1}^2}

\newcommand{\pnorm}[2]{\norm{#2}_{#1}}
\newcommand{\infnorm}[1]{\norm{#1}_{\infty}}

\newcommand{\iinorm}[1]{\pnorm{\infty,\infty}{#1}}

\newcommand{\dist}{\operatorname{dist}}

\newcommand{\triplenorm}[1]{\left\vert\!\left\vert\!\left\vert {#1} \right\vert\!\right\vert\!\right\vert}

\newcommand{\opnorm}[1]{\ensuremath{\triplenorm{#1}}}

%%% Optimization

% Minimization program
\newcommand{\minprog}[3]{
  \left.
  \begin{array}{ll}
    \text{minimize}_{#1} & {#2}  \\[5pt]
    \text{subject to} & #3
  \end{array}
  \right.
}

%%% Landau notation
\newcommand{\bigOh}{\mathcal{O}}

%%% Special definitions for inliers/outliers
\newcommand{\In}{\ensuremath{\mathrm{In}}}
\newcommand{\Out}{\ensuremath{\mathrm{Out}}}
\newcommand{\Xin}{\ensuremath{\mathcal{X}_{\mathrm{In}}}}
\newcommand{\Xout}{\ensuremath{\mathcal{X}_{\mathrm{Out}}}}
\newcommand{\Xall}{\ensuremath{\mathcal{X}}}

\newcommand{\Expr}{\ensuremath{\mathcal{E}}}
\newcommand{\sExpr}{\ensuremath{\tilde{\mathcal{E}}}}
\newcommand{\Strct}{\ensuremath{\mathcal{S}}}
\newcommand{\sStrct}{\ensuremath{\tilde{\mathcal{S}}}}
%%% Special definitions for inliers/outliers

%\newcommand{\Xin}{\ensuremath{\mathcal{X}_{\mathrm{In}}}}
%\newcommand{\Xout}{\ensuremath{\mathcal{X}_{\mathrm{Out}}}}

\newcommand{\bx}{\boldsymbol{x}}
\newcommand{\bs}{\boldsymbol{s}}
\newcommand{\bT}{\boldsymbol{T}}
\newcommand{\bW}{\boldsymbol{W}}
\newcommand{\bw}{\boldsymbol{w}}
\newcommand{\by}{\boldsymbol{y}}
\newcommand{\bZ}{\boldsymbol{Z}}
\newcommand{\bc}{\boldsymbol{c}}
\newcommand{\bz}{\boldsymbol{z}}
\newcommand{\bX}{\boldsymbol{X}}
\newcommand{\bE}{\boldsymbol{E}}
\newcommand{\bF}{\boldsymbol{F}}
\newcommand{\bL}{\boldsymbol{L}}
\newcommand{\bN}{\boldsymbol{N}}
\newcommand{\bO}{\boldsymbol{O}}
\newcommand{\bP}{\boldsymbol{P}}
\newcommand{\bQ}{\boldsymbol{Q}}
\newcommand{\bD}{\boldsymbol{D}}
\newcommand{\bbeta}{\boldsymbol{\beta}}
\newcommand{\sX}{\mathcal{X}}
\newcommand{\sA}{\mathcal{A}}
\newcommand{\sY}{\mathcal{Y}}
\newcommand{\bSigma}{\boldsymbol\Sigma}
\newcommand{\bDelta}{\boldsymbol\Delta}
\newcommand{\bU}{\boldsymbol{U}}
\newcommand{\bV}{\boldsymbol{V}}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}


\def\reals{\mathbb{R}}
\def\E{\mathbb{E}}
\def\bd{\boldsymbol{d}}

\def\bx{\boldsymbol{x}}
\def\bga{\boldsymbol{\gamma}}
\def\beps{\boldsymbol{\epsilon}}
\def\be{\boldsymbol{e}}
\def\bt{\boldsymbol{t}}
\def\bu{\boldsymbol{u}}
\def\bS{\boldsymbol{S}}
\def\bLam{\boldsymbol{\Lambda}}
\def\b0{\mathbf{0}}
\def\bzero{\boldsymbol{0}}

\def\bP{\boldsymbol{P}}
\def\bQ{\boldsymbol{Q}}
%\def\bC{\boldsymbol{C}}
\def\bSigma{\boldsymbol\Sigma}
\def\bGamma{\boldsymbol\Gamma}
\def\bDelta{\boldsymbol\Delta}
\def\bU{\boldsymbol{U}}
\def\bR{\boldsymbol{R}}
\def\bC{\boldsymbol{C}}
\def\bv{\boldsymbol{v}}
\def\bA{\boldsymbol{A}}
\def\bY{\boldsymbol{Y}}
\def\bh{\boldsymbol{h}}
\def\br{\boldsymbol{r}}
\def\bB{\boldsymbol{B}}
\def\bg{\boldsymbol{g}}
\def\bH{\boldsymbol{H}}
\def\bn{\boldsymbol{n}}
\def\calD{\mathcal{D}}
\def\bI{\boldsymbol{I}}
\def\TV{\mathrm{TV}}
\def\im{\mathrm{im}}
\def\tr{\mathrm{tr}}
\def\rmL{\mathrm{L}}
\def\rmV{\mathrm{V}}
\def\Nin{N_{\text{in}}}
\def\Nout{N_{\text{out}}}
\def\SPSD{\mathrm{S_+}}
\def\CTF{\mathrm{CTF}}
\def\nnz{\mathsf{nnz}}

\newcommand{\bSig}{\boldsymbol{\Sigma}}

\newcommand{\Cov}{\text{Cov}}
\newcommand{\Var}{\text{Var}}
\newcommand{\bmu}{\boldsymbol{\mu}}
\newcommand{\bo}{\boldsymbol{0}}



\def\orth{\mathrm{orth}}
\def\PSD{\mathrm{S_{++}}}
\def\Sp{\mathrm{Sp}}
\def\HPSD{\mathbb{H}}
\def\bbH{\mathbb{H}}
\newcommand{\di}{{\,\mathrm{d}}}
\newcommand{\iu}{{i\mkern1mu}} 
